Privacy Policy Analysis through Prompt Engineering for LLMs

Privacy policies are often obfuscated by their complexity, which impedes transparency and informed consent. Conventional machine learning approaches for automatically analyzing these policies demand significant resources and substantial domain-specific training, causing adaptability issues. Moreover, they depend on extensive datasets that may require regular maintenance due to changing privacy concerns. In this paper, we propose, apply, and assess PAPEL (Privacy Policy Analysis through Prompt Engineering for LLMs), a framework harnessing the power of Large Language Models (LLMs) through prompt engineering to automate the analysis of privacy policies. PAPEL aims to streamline the extraction, annotation, and summarization of information from these policies, enhancing their accessibility and comprehensibility without requiring additional model training. By integrating zero-shot, one-shot, and few-shot learning approaches and the chain-of-thought prompting in creating predefined prompts and prompt templates, PAPEL guides LLMs to efficiently dissect, interpret, and synthesize the critical aspects of privacy policies into user-friendly summaries. We demonstrate the effectiveness of PAPEL with two applications: (i) annotation and (ii) contradiction analysis. We assess the ability of several LLaMa and GPT models to identify and articulate data handling practices, offering insights comparable to existing automated analysis approaches while reducing training efforts and increasing the adaptability to new analytical needs. The experiments demonstrate that the LLMs PAPEL utilizes (LLaMA and Chat GPT models) achieve robust performance in privacy policy annotation, with F1 scores reaching 0.8 and above (using the OPP-115 gold standard), underscoring the effectiveness of simpler prompts across various advanced language models.

==> Results/table_consistency.tex <==
%\begin{table}[h]
%\caption{Caption}
\begin{wraptable}[]{t}{0.560\linewidth}
\vspace*{-1.30em}
    %\centering
    \caption{Caption???}
\scriptsize
\newcolumntype{t}{>{\tiny}c}
\label{tab:consistency}
\vspace*{-1.5em}
\begin{tabular}{c|ct|c|}
                     & \multicolumn{2}{c|}{\textbf{Consistency}}                                                         \\
                     & \textbf{avg  F1\textsubscript{cons}} & \textbf{Exactly  equal [\%]} \\ \hline
\textbf{LlaMA-2 7B}  & 0.89                                                        & 70.7                       \\
\textbf{LlaMA-2 70B} &                                                         &                           \\
\textbf{LlaMA-3 8B} &  0.84                                                     & 53.4                       \\
\textbf{LlaMA-3 70B} & 0.83                                                        & 48.2                           \\
\textbf{GPT 3.5}     & 0.94                                                         & 72.6                       \\
\textbf{GPT 4}       & 0.98                                                         & 81.2                       \\
\textbf{GPT 4 Turbo} & 0.97                                                         & 83.1                      
\end{tabular}
\vspace*{-1.30em}
\end{wraptable}

==> Results/table_prompts_gpt4.tex <==
%\begin{table}[hb]
\begin{table*}[t]
%\small
\scriptsize
\caption{F1 performance with confidence intervals for Chat GPT 4 engine given different prompts. The micro average F1 score is highlighted to facilitate comparison with performance quoted in the literature.}
\vspace*{-1.0em}
\newcolumntype{t}{>{\tiny}p{0.02\textwidth}}
\newcolumntype{n}{>{\centering}p{0.075\textwidth}}
\newcolumntype{o}{>{\centering}p{0.08\textwidth}}
\newcolumntype{s}{>{\centering}p{0.04\textwidth}}
\begin{tabular}{l|st|st|st|}
\multicolumn{1}{c|}{\multirow{2}{*}{\textbf{GPT 4}}} & \multicolumn{2}{o|}{\textbf{Prompt I}}                                  & \multicolumn{2}{o|}{\textbf{Prompt II}}                              & \multicolumn{2}{o|}{\textbf{Prompt III}}                             \\
\multicolumn{1}{c|}{}                                & \multicolumn{1}{c}{\textbf{F1}} & \multicolumn{1}{c|}{\textbf{±}} & \multicolumn{1}{c}{\textbf{F1}} & \multicolumn{1}{c|}{\textbf{±}} & \multicolumn{1}{c}{\textbf{F1}} & \multicolumn{1}{c|}{\textbf{±}} \\ \hline
\textbf{User Choice/Ctrl}                         & 0.58                                  & 0.06                            & 0.61                               & 0.06                            & 0.62                               & 0.06                            \\
\textbf{1\textsuperscript{st} Party Collection}                  & 0.85                                  & 0.02                            & 0.87                               & 0.02                            & 0.87                               & 0.02                            \\
\textbf{3\textsuperscript{rd} Party Sharing}              & 0.84                                  & 0.03                            & 0.85                               & 0.03                            & 0.84                               & 0.03                            \\
\textbf{Do Not Track}                                & 0.93                                  & 0.09                            & 0.93                               & 0.10                            & 0.93                               & 0.10                            \\
\textbf{Access, Edit \& Del}              & 0.63                                  & 0.07                            & 0.64                               & 0.07                            & 0.69                               & 0.07                            \\
\textbf{Data Security}                               & 0.80                                  & 0.06                            & 0.77                               & 0.06                            & 0.78                               & 0.05                            \\
\textbf{Data Retention}                              & 0.61                                  & 0.14                            & 0.59                               & 0.14                            & 0.66                               & 0.15                            \\
\textbf{Specific   Audiences}      & 0.76                                  & 0.06                            & 0.87                               & 0.05                            & 0.90                               & 0.04                            \\
\textbf{Policy Change}                               & 0.87                                  & 0.05                            & 0.86                               & 0.05                            & 0.87                               & 0.05                            \\ \hline
\textbf{micro avg}                                   & 0.78                        & 0.02                            & 0.80                     & 0.02                            & 0.81                     & 0.02                            \\
%\textbf{macro avg}                                   & 0.76                                  & 0.02                            & 0.78                               & 0.02                            & 0.80                               & 0.02                            \\
%\textbf{weighted avg}                                & 0.79                                  & 0.02                            & 0.82                               & 0.02                            & 0.82                               & 0.02                            \\
%\textbf{samples avg}                                 & 0.82                                  & 0.02                            & 0.85                               & 0.02                            & 0.85                               & 0.01                           
\end{tabular}
\label{tab:result_prompts}
\end{table*}

==> prompts.tex <==
\section{Prompt Engineering for Policy Analysis}
\label{sec:prompts}

\subsection{Prompt I: Data category title}

Websites and digital products have privacy policies. I will give you a dataset of privacy policies, where privacy policies are divided into paragraph length segments and each segment is annotated with one or more data practice. A data practice means how the data is used and processed by an organization. In current context, a data practice belongs to one of the following data practice category. 
 
1. First Party Collection/Use.
2. Third Party Sharing/Collection.
3. User Choice/Control.
4. User Access, Edit, and Deletion.
5. Data Retention.
6. Data Security. 
7. Policy Change.
8. Do Not Track.
9. International and Specific Audiences.
10. Other.
 
I have a specific task for you: The user will give you a sentence from some privacy contents, and you tell them which category of practices this sentence may contain. Please only respond with the category.


\subsection{Prompt II: Data category title with OPP-115 description}

Websites and digital products have privacy policies. I will give you a dataset of privacy policies, where privacy policies are divided into paragraph length segments and each segment is annotated with one or more data practice. A data practice means how the data is used and processed by an organization. In current context, a data practice belongs to one of the following data practice category. 
 
1. First Party Collection/Use: how and why a service provider collects user information.
2. Third Party Sharing/Collection: how user information may be shared with or collected by
third parties.
3. User Choice/Control: choices and control options available to users.
4. User Access, Edit, and Deletion: if and how users may access, edit, or delete their information.
5. Data Retention: how long user information is stored.
6. Data Security: how user information is protected.
7. Policy Change: if and how users will be informed about changes to the privacy policy.
8. Do Not Track: if and how Do Not Track signals for online tracking and advertising are
honored.
9. International and Specific Audiences: practices that pertain only to a specific group of users (e.g., children, Europeans, or California residents).
10. Other: additional sub-labels for introductory or general text, contact information, and
practices not covered by the other categories.
 
I have a specific task for you: The user will give you a sentence from some privacy contents, and you tell them which category of practices this sentence may contain. Please only respond with the category.

\subsection{Prompt III: Data category title with extended description}
Websites and digital products have privacy policies. I will give you a dataset of privacy policies, where privacy policies are divided into paragraph length segments and each segment is annotated with one or more data practice. A data practice means how the data is used and processed by an organization. In current context, a data practice belongs to one of the following data practice category. 
 
1. First Party Collection/Use: how and why a service provider collects user information. In first party collection the service provider that owns or operates the website/platform/service directly collect data from individuals. 
2. Third Party Sharing/Collection: how user information may be shared with or collected by
third parties. In third party sharing/collection an entity other than the service provider collects data from users through the service provider's platform. Third parties could include advertisers, analytic companies, or partner services that have their own data collection and privacy practices.
3. User Choice/Control: choices and control options available to users. Choice means giving individuals options as to how their personal information may be used. Specifically, choice relates to secondary uses of information—that is, uses beyond those necessary to complete the contemplated transaction. Control means privacy controls that allow individuals to manage use and sharing of their data. 
4. User Access, Edit, and Deletion: if and how users may access, edit, or delete their information.
5. Data Retention: how long user information is stored. All data should have retention period associated with it, retention period means maximum period the data will be stored. 
6. Data Security: how user information is protected. In particular, it means the security measures that ensures security of personal data, including encryption or storage of data on secure servers. 
7. Policy Change: if and how users will be informed about changes to the privacy policy.
8. Do Not Track: if and how Do Not Track signals for online tracking and advertising are
honored.
9. International and Specific Audiences: practices that pertain only to a specific group of users (e.g., children, Europeans, or California residents).
10. Other: additional sub-labels for introductory or general text, contact information, and
practices not covered by the other categories.


\subsection{Prompt IV: Data category title with extended description and examples}

